First observation and measurement of the branching fraction for the decay $B^0_s \to D_s^{*\mp} K^{\pm}$

The first observation of the $B^0_s \to D_s^{*\mp} K^{\pm}$ decay is reported using 3.0$fb^{-1}$ of proton-proton collision data collected by the LHCb experiment. The $D_s^{*\mp}$ mesons are reconstructed through the decay chain $D_s^{*\mp} \to \gamma D_s^{\mp}(K^{\mp}K^{\pm}\pi^{\mp})$. The branching fraction relative to that for $B^0_s \to D_s^{*-} \pi^{+}$ is measured to be $0.068 \pm 0.005 ^{+0.003}_{-0.002}$, where the first uncertainty is statistical and the second is systematic. Using a recent measurement of $BR(B^0_s \to D_s^{*-} \pi^{+})$ the absolute branching fraction of $B^0_s \to D_s^{*\mp} K^{\pm}$ is measured as ( 16.3 $\pm$ 1.2 (stat) $^{+0.7}_{-0.5}$ (syst) $\pm$ 4.8 (norm) ) $\times$ 10$^{-5}$, where the third uncertainty is due to the uncertainty on the branching fraction of the normalisation channel.

==> tikz.tex <==
%Feynman diagrams Bs->Ds-K+
\begin{figure}[!htb]
  \begin{center}
	\begin{tikzpicture}[thick,scale=1.3]
		\draw               (0,0) .. controls (-.2, .5) .. (0,1) node[midway,left=4pt] {\Bs};
		\draw               (0,0) .. controls ( .2, .5) .. (0,1);
		\draw[antiparticle] (0,1) -- node[black,above=4pt,sloped] {\bquarkbar} (1,1);
		\draw               (1,1) -- (2,1);
		\draw[antiparticle] (2,1) -- node[black,above=4pt] {\cquarkbar} (3,1);
		\draw[particle]     (0,0) -- node[black,below=4pt,sloped] {\squark} (3,0);
		\draw               (3,0) .. controls ( 2.8, .5) .. (3,1);
		\draw               (3,0) .. controls ( 3.2, .5) .. (3,1) node[midway,right=4pt] {\Dssm};

		\draw[boson]        (1.5,1) -- node[black,left=4pt] {\Wp} (2,2.5);

		\draw               (3,3) .. controls (2.8, 2.5) .. (3,2);
		\draw               (3,3) .. controls (3.2, 2.5) .. (3,2) node[midway,right=4pt] {\Kp};
		\draw[particle]     (2,2.5) -- node[black,above=4pt] {\uquark} (3,3);
		\draw[antiparticle] (2,2.5) -- node[black,below=4pt] {\squarkbar} (3,2);
	\end{tikzpicture}
	\begin{tikzpicture}[thick,scale=1.3]
		\draw               (0,0) .. controls (-.2, .5) .. (0,1) node[midway,left=4pt] {\Bs};
		\draw               (0,0) .. controls ( .2, .5) .. (0,1);
		\draw[antiparticle] (0,1) -- node[black,above=4pt,sloped] {\bquarkbar} (1,1);
		\draw               (1,1) -- (2,1);
		\draw[antiparticle] (2,1) -- node[black,above=4pt] {\uquarkbar} (3,1);
		\draw[particle]     (0,0) -- node[black,below=4pt,sloped] {\squark} (3,0);
		\draw               (3,0) .. controls ( 2.8, .5) .. (3,1);
		\draw               (3,0) .. controls ( 3.2, .5) .. (3,1) node[midway,right=4pt] {\Km};

		\draw[boson]        (1.5,1) -- node[black,left=4pt] {\Wp} (2,2.5);

		\draw               (3,3) .. controls (2.8, 2.5) .. (3,2);
		\draw               (3,3) .. controls (3.2, 2.5) .. (3,2) node[midway,right=4pt] {\Dssp};
		\draw[particle]     (2,2.5) -- node[black,above=4pt] {\cquark} (3,3);
		\draw[antiparticle] (2,2.5) -- node[black,below=4pt] {\squarkbar} (3,2);
	\end{tikzpicture}
  \end{center}
  \caption{\small
    Feynman diagrams of the first-order contributions to the processes \decay{\Bs}{\Dssm\Kp} (left) and \decay{\Bs}{\Dssp\Km} (right).}
  \label{fig:BsDsKFeynmanDiagram}
\end{figure}

%Feynman diagrams Bs->Ds-Pi+, Bd->Ds-K+
\begin{figure}[!htb]
  \begin{center}
	\begin{tikzpicture}[thick,scale=1.3]
		\draw               (0,0) .. controls (-.2, .5) .. (0,1) node[midway,left=4pt] {\Bs};
		\draw               (0,0) .. controls ( .2, .5) .. (0,1);
		\draw[antiparticle] (0,1) -- node[black,above=4pt,sloped] {\bquarkbar} (1,1);
		\draw               (1,1) -- (2,1);
		\draw[antiparticle] (2,1) -- node[black,above=4pt] {\cquarkbar} (3,1);
		\draw[particle]     (0,0) -- node[black,below=4pt,sloped] {\squark} (3,0);
		\draw               (3,0) .. controls ( 2.8, .5) .. (3,1);
		\draw               (3,0) .. controls ( 3.2, .5) .. (3,1) node[midway,right=4pt] {\Dssm};

		\draw[boson]        (1.5,1) -- node[black,left=4pt] {\Wp} (2,2.5);

		\draw               (3,3) .. controls (2.8, 2.5) .. (3,2);
		\draw               (3,3) .. controls (3.2, 2.5) .. (3,2) node[midway,right=4pt] {\pip};
		\draw[particle]     (2,2.5) -- node[black,above=4pt] {\uquark} (3,3);
		\draw[antiparticle] (2,2.5) -- node[black,below=4pt] {\dquarkbar} (3,2);
	\end{tikzpicture}
	\begin{tikzpicture}[thick,scale=1.3]
		\draw               (0,0) .. controls (-.2, .5) .. (0,1) node[midway,left=4pt] {\Bs};
		\draw               (0,0) .. controls ( .2, .5) .. (0,1);
		\draw[antiparticle] (0,1) -- node[black,above=4pt,sloped] {\bquarkbar} (1,1);
		\draw[particle]     (0,0) -- node[black,below=4pt,sloped] {\dquark} (1,0);

		\draw[boson]        (1,1) -- node[black,left=2pt] {\Wp} (1,0);

        \draw[particle]     (1.5,0.5) -- node[black,below=4pt] {\squark} (2,1);
		\draw[antiparticle] (1,1) -- node[black,above=4pt] {\cquarkbar} (2,2);
		\draw               (2,1) .. controls (1.8, 1.5) .. (2,2);
		\draw               (2,1) .. controls (2.2, 1.5) .. (2,2) node[midway,right=4pt] {\Dssm};

        \draw[gluon]        (1.2,1.2) -- node[black,below=5pt] {\Pg} (1.5,0.5);

		\draw[particle]     (1,0) -- node[black,below=4pt] {\uquark} (2,-1);
        \draw[antiparticle] (1.5,0.5) -- node[black,below=4pt] {\squarkbar} (2,0);
		\draw               (2,0) .. controls (1.8, -0.5) .. (2,-1);
		\draw               (2,0) .. controls (2.2, -0.5) .. (2,-1) node[midway,right=4pt] {\Kp};
	\end{tikzpicture}
  \end{center}
  \caption{\small
    Feynman diagrams of the first-order contributions to the processes \Bs $\to$ \Dssm \pip (left) and 
    \decay{\Bz}{\Dssm\Kp} (right).}
  \label{fig:BsDsPiBdDsKFeynmanDiagram}
\end{figure}

